LiVLR: A Lightweight Visual-Linguistic Reasoning Framework for Video Question Answering

Video Question Answering (VideoQA), aiming to correctly answer the given question based on understanding multi-modal video content, is challenging due to the rich video content. From the perspective of video understanding, a good VideoQA framework needs to understand the video content at different semantic levels and flexibly integrate the diverse video content to distill question-related content. To this end, we propose a Lightweight Visual-Linguistic Reasoning framework named LiVLR. Specifically, LiVLR first utilizes the graph-based Visual and Linguistic Encoders to obtain multi-grained visual and linguistic representations. Subsequently, the obtained representations are integrated with the devised Diversity-aware Visual-Linguistic Reasoning module (DaVL). The DaVL considers the difference between the different types of representations and can flexibly adjust the importance of different types of representations when generating the question-related joint representation, which is an effective and general representation integration method. The proposed LiVLR is lightweight and shows its performance advantage on two VideoQA benchmarks, MRSVTT-QA and KnowIT VQA. Extensive ablation studies demonstrate the effectiveness of LiVLR key components.

==> figure/visualization.tex <==
\begin{figure*}[!tbp]
\begin{center}
\includegraphics[width=0.5\linewidth]{figure/vis_gs1.pdf}
\end{center}
\vspace{-2mm}
\caption{Prediction examples on MSRVTT-QA~\cite{xu2017video}. 
$\ModelName$ utilizes $\ModuleName$ and RI-GCN as the representation integration (RI) methods, respectively. 
Compared with RI-GCN, which is the existing best RI method in the VideoQA task, the proposed $\ModuleName$ performs better in handle multi-grained questions corresponding to the same video clip, demonstrating the effectiveness of $\ModuleName$. 
}
\label{fig:vis_gs}
\end{figure*}

\begin{figure*}[tbp]
\begin{center}
\includegraphics[width=1.0\linewidth]{figure/vis_ss.pdf}
\end{center}
\caption{Prediction examples on MSRVTT-QA~\cite{xu2017video}. 
$\ModelName$ utilizes $\ModuleName$ and RI-GCN as the RI methods, respectively. 
Compared with RI-GCN, the proposed $\ModuleName$ performs better in answering multi-source questions, demonstrating that $\ModuleName$ is an effective RI method.  
}
\label{fig:vis_ss}
\end{figure*}


\begin{figure*}[tbp]
\begin{center}
\includegraphics[width=1.0\linewidth]{figure/error.pdf}
\end{center}
\caption{Prediction examples on MSRVTT-QA~\cite{xu2017video}. 
$\ModelName$ utilizes $\ModuleName$ and RI-GCN as the RI methods, respectively. 
Compared with RI-GCN, the proposed $\ModuleName$ performs better in answering multi-source questions, demonstrating that $\ModuleName$ is an effective RI method.  
}
\label{fig:vis_error}
\end{figure*}


\begin{figure*}[!thp]
\begin{center}
\includegraphics[width=1.0\linewidth]{figure/correlation.pdf}
\end{center}
\caption{Prediction examples on MSRVTT-QA~\cite{xu2017video}. 
$\ModelName$ utilizes $\ModuleName$ and RI-GCN as the RI methods, respectively. 
Compared with RI-GCN, the proposed $\ModuleName$ performs better in answering multi-source questions, demonstrating that $\ModuleName$ is an effective RI method.  
}
\label{fig:vis_correlation}
\end{figure*}


==> section/sup.tex <==
% % **********************************************************************
% \section{Details of Feature Extraction}
% \label{sec:data_preprocess} 
% To obtain the inputs of $\ModelName$ (\ie, the visual and linguistic features), we utilize ResNet-101~\cite{he2016deep} pre-trained on ImageNet~\cite{deng2009imagenet} to extract the holistic image appearance features for the three experimental datasets, and use bottom-up attention Faster R-CNN~\cite{anderson2018bottom} pre-trained on Visual Genome~\cite{krishna2017visual} to detect objects and corresponding class-attributes in each sampled image. 
% More specifically, for MSRVTT-QA, we sampled 64 frames at an equal interval from each video clip, and 12 sentences as the linguistic sentences for each video clip from the provided caption annotations in~\cite{xu2016msr}. The number of detected objects in each sampled image is 10. 
% For KnowIT VQA, the number of sampled images and detected objects are 32 and 12, respectively. We use the provided reason condensed from subtitles of video as the linguistic sentences. 
% For TVQA, the number of sampled images is $N_f=32$, and the detected objects number is $N_o=12$. 
% We use subtitles provided by TVQA~\cite{lei2018tvqa} to generate linguistic representations. 


% **********************************************************************
\section{Ablation Study on Hyperparameter} 

\subsection{Question-related Attention} 
\label{sec:QAtt} 
The Question-related Attention block ($\mathcal{Q}_{\text{att}}$) is employed to associate the multi-grained and multi-source representations ($\Xmat_{V, g}, \Xmat_{V, l}, \Xmat_{L, g}, \Xmat_{L, l}$) to the question-related representation ($\Qmat$). This is significant to distill the question-related information from multi-grained and multi-source information. Therefore, we execute some ablations to analyze the key hyperparameter $N_h$ in $\mathcal{Q}_{\text{att}}$. 
Specifically, we consider following settings: $N_h = 1, 4, 8, 16, 32$. 
From the experimental results in Table~\ref{tab:abl_params}, we observe that, compared with the overall performance improvement, the performance fluctuation of $\ModelName$ using different $N_h$ is slight, demonstrating that our method is robust to the hyperparameter $N_h$. 

% *********************************************************************
\input{table/abl_parameter.tex} 
% *********************************************************************

\subsection{Linguistic Embedding}
\label{sec:LE}

There are two prevailing methods for embedding linguistic sentences into feature vectors in the $\Problem$ task: BERT~\cite{devlin2018bert} and GloVe~\cite{pennington2014glove}. 
To illustrate the effectiveness of the proposed $\ModelName$ with the two kinds of linguistic embeddings as inputs, we validate it on MSRVTT-QA and KnowIT-VQA. 
Results in Table~\ref{tab:abl_params} show that the proposed $\ModelName$ is robust to different types of linguistic embedding input. 

\input{figure/visualization.tex}

\section{Qualitative Examples}
\label{sec:visualization}
To qualitatively analyze the effectiveness of the proposed $\ModuleName$ for representation integration (RI), we visualize some prediction examples on MSRVTT-QA~\cite{xu2017video} in \figurename~\ref{fig:vis_gs} and \figurename~\ref{fig:vis_ss}. 
RI-GCN is the existing best RI method in the VideoQA task. 
Compared with RI-GCN, the proposed $\ModuleName$ performs better in handling multi-grained questions corresponding to the same video clip (Figure~\ref{fig:vis_gs}) and multi-source questions (Figure~\ref{fig:vis_ss}), demonstrating that $\ModuleName$ is an effective RI method. 




==> table/abl_parameter.tex <==
\begin{table}[!thbp]
\begin{center}
\small
\setlength{\tabcolsep}{1.1mm}{
\caption{Ablation studies on the hyperparameter $N_h$ and the Linguistic Embedding type (LE).  
}
\label{tab:abl_params}
\vspace{-2mm}
\begin{tabular}{c|c|c|c}
\hline
&\#Variable &MSRVTT-QA~\cite{xu2017video} &KnowIT-VQA~\cite{garcia2020knowit} \\ 
\hline
\hline
% \multirow{6}{*}{$N_h$} &w/o &49.72 &74.73 \\ 
\multirow{5}{*}{$N_h$} &1 &57.83 &76.83 \\
&4 &58.61 &77.00 \\
&8 &59.30 &\textbf{77.10} \\
&16 &\textbf{59.44} &76.95 \\
&32 &59.09 &76.91 \\
% \hline
% % \hline
% \multirow{2}{*}{LE} &BERT &\textbf{59.44} &\textbf{77.10} \\
% &GloVe &57.23 &76.23 \\
% \hline
% \rowcolor{gray!15}SoTA &--- &\multicolumn{1}{c|}{35.60} &\multicolumn{1}{c}{73.10} \\
\hline
\end{tabular}
} % scale box
\end{center}
\end{table}

% \begin{table}[!t]
% \begin{center}
% \centering
% \small
% \setlength{\tabcolsep}{1.1mm}{
% % \renewcommand\arraystretch{1.1}
% \begin{tabular}{c|c|c|c}
% \hline
% &\#Variable &MSRVTT-QA~\cite{xu2017video} &KnowIT-VQA~\cite{garcia2020knowit} \\ 
% \hline
% \hline
% % \multirow{6}{*}{$N_h$} &w/o &49.72 &74.73 \\ 
% \multirow{5}{*}{$N_h$} &1 &57.83 &76.83 \\
% &4 &58.61 &77.00 \\
% &8 &59.30 &\textbf{77.10} \\
% &16 &\textbf{59.44} &76.95 \\
% &32 &59.09 &76.91 \\
% \hline
% % \hline
% \multirow{2}{*}{LE} &BERT &\textbf{59.44} &\textbf{77.10} \\
% &GloVe &57.23 &76.23 \\
% \hline
% \rowcolor{gray!15}SoTA &- &\multicolumn{1}{c|}{35.60} &\multicolumn{1}{c}{73.10} \\
% \hline
% \end{tabular}
% } % scale box
% \end{center}
% \vspace{-1mm}
% \caption{Ablation studies on the hyperparameter $N_h$ and the Linguistic Embedding (LE) type. Compared with the existing state-of-the-art (SoTA) performance, the overall performance improvements demonstrate that our $\ModelName$ is robust to $N_h$ and LE. 
% }
% \label{tab:abl_params}
% \end{table}

% \begin{table}[!t]
% \begin{center}
% \small
% \resizebox{1.0\linewidth}{!}{
% \renewcommand\arraystretch{1.1}
% \begin{tabular}{c|c|c}
% \hline
% \#Variable ($N_h$) &MSRVTT-QA~\cite{xu2017video} &KnowIT-VQA~\cite{garcia2020knowit} \\ 
% \hline
% \hline
% w/o &49.72 &74.73 \\ 
% 1 &57.83 &76.83 \\
% 4 &58.61 &77.00 \\
% 8 &59.30 &\textbf{77.10} \\
% 16 &\textbf{59.44} &76.95 \\
% 32 &59.09 &76.91 \\
% \hline
% % \hline
% \rowcolor{gray!10}SoTA &\multicolumn{1}{c|}{35.6} &\multicolumn{1}{c}{73.1} \\
% \hline
% \end{tabular}
% } % scale box
% \end{center}
% \vspace{-1mm}
% \caption{Accuracies (\%) on MRSVTT-QA and KnowIT-VQA of different hyperparameter settings. The last row reports the existing state-of-the-art (SoTA) performance on the two benchmarks.}
% \label{tab:abl_params}
% \end{table}

% ***********************************************************************
% \begin{table}[tbp]
% \begin{center}
% % \small
% \resizebox{0.9\linewidth}{!}{
% \renewcommand\arraystretch{1.1}
% \footnotesize
% \begin{tabular}{c|c|c|c|c}
% \hline
% \multirow{2}{*}{Acc. ($\%$)} 
% &\multicolumn{2}{c|}{MSRVTT-QA~\cite{xu2017video}} 
% &\multicolumn{2}{c}{KnowIT-VQA~\cite{garcia2020knowit}} 
% \\
% \cline{2-5}
% &BERT &GloVe &BERT &GloVe \\
% \hline
% \hline
% &\textbf{59.44} &57.23 &\textbf{77.10} &76.23 \\
% \hline
% \end{tabular}
% } % scale box
% \end{center}
% \vspace{-1mm}
% \caption{Experimental results of $\ModelName$ using different types of linguistic feature extraction. }
% \label{tab:abl_lf_extraction}
% \end{table}

% ***********************************************************************



